CrowdProve: Community Proving for ZK Rollups

Zero-Knowledge (ZK) rollups have become a popular solution for scaling blockchain systems, offering improved transaction throughput and reduced costs by aggregating Layer 2 transactions and submitting them as a single batch to a Layer 1 blockchain. However, the computational burden of generating validity proofs, a key feature of ZK rollups, presents significant challenges in terms of performance and decentralization. Current solutions rely on centralized infrastructure to handle the computational tasks, limiting the scalability and decentralization of rollup systems. This paper proposes CrowdProve, a prover orchestration layer for outsourcing computation to unreliable commodity hardware run by a broad community of small provers. We apply CrowdProve to proving transaction batches for a popular ZK rollup. Through our experimental evaluation, we demonstrate that community proving can achieve performance comparable to, and in some cases better than, existing centralized deployments. Our results show that even systems utilizing modest hardware configurations can match the performance of centralized solutions, making community-based proof generation a viable and cost-effective alternative. CrowdProve allows both the rollup operator and community participants to benefit: the operator reduces infrastructure costs by leveraging idle community hardware, while community provers are compensated for their contributions.

==> 1_intro.tex <==
\section{Introduction}
Rollups have become a very popular way of scaling blockchain systems. A rollup (such as ZKsync)
is a transaction processing system built on top of another blockchain system (such as Ethereum).
That is why we refer to the rollup as being at ``level 2''~(L2) with respect to its associated blockchain system defined to be at ``level 1''~(L1).
While the L1 system usually offers very strong safety and liveness guarantees and is decentralized and Sybil-resistant,
it tends to sacrifice performance (transaction latency and throughput).
Moreover, low throughput easily induces contention that leads to high transaction fees on the L1.
The rollup's purpose is to order and execute transactions submitted to it (L2 transactions) faster and cheaper than the L1 system.
Periodically, the rollup submits only the result of executing a large batch of L2 transactions to the L1 system as a single L1 transaction, amortizing the associated cost over all the L2 transactions in the batch.

Fast and cheap execution at a rollup is usually enabled at the expense of decentralization.
The ordering and execution of rollup transactions is often performed by a single centralized sequencer.
To ensure the correctness of the execution despite a potentially malicious rollup operator, there exist two established approaches:
\begin{enumerate}
    \item with \emph{fraud proofs}, used by optimistic rollups, anyone is able to re-execute the transactions and check for inconsistencies that would lead to punishing a misbehaving rollup operator.
    \item with \emph{validity proofs}, used by ZK rollups, the rollup operator uses zero-knowledge cryptographic techniques
    to generate an easy-to-verify proof of correctness of the execution. The validity proof is then checked directly by a smart contract on the L1 chain,
    providing instant guarantee of the correctness of the execution result.
\end{enumerate}
This paper is uniquely concerned with ZK rollups, more specifically, with the computation of validity proofs and a path towards its decentralization.

Generating a validity proof tends to require a large amount of computation -- orders of magnitude more than the execution of the transactions itself.
It involves a variety of different computational tasks with different hardware requirements. Depending on the used proof system, some are demanding in computation, some have a large memory footprint, some are highly parallelizable, and some can be efficiently accelerated with GPUs. Moreover, the results of some are easily verifiable (as they are proofs themselves) while the results of others are not. All those (and many more) considerations are important for decentralizing the proof generation.

Instead of trying to fully decentralize the generation of the proof, we propose a \emph{partial} decentralization, where some, but not all, proving sub-tasks are performed by the public / the community, while others remain reserved to the rollup operator. The insight is that with a relatively low effort, one can achieve partial decentralization by only outsourcing the tasks for which doing so is easy.

It is important to note that, technically, a system is centralized as long as any single of its essential components is centralized. In this sense, full control over the proving remains in the hands of the rollup operator who merely outsources certain tasks to the public. Nevertheless, this approach presents the first step in the right direction.
In order to achieve true decentralization, the orchestration of the proving process would also need to be performed by a decentralized system, such as a smart contract (discussed in Section~\ref{sec:discussion}).
However, our solution is beneficial for both
\begin{enumerate}
    \item community participants who earn rewards for employing their hardware that might otherwise be idle and
    \item the rollup operator who, by outsourcing certain tasks, saves on infrastructure cost, assuming that community participants are ready to offer a lower price than the price of using the rollup operator’s own (or rented) hardware.
\end{enumerate}

We propose such a partially distributed proving system for the Boojum prover used by ZKsync.
We modify the system in a way to enable anyone with a sufficiently performant computer to participate in the proving process.
The performance requirements are easily met by a regular personal computer.
Moreover, our system makes sure that even a misbehaving prover is unable to disrupt the system.
While our concrete implementation is Boojum-specific, our design stays general and its principles can be applied to other proving system implementations as well.

Outsourcing computational tasks to community provers brings about new challenges compared to a centralized approach.
The most prominent one is that public provers cannot be fully trusted by the system.
One always needs to assume that they may fail, for example by producing incorrect results or no results at all.
Such faults must be dealt with, ideally without a severe impact on the overall system performance or running cost.
Fortunately, there are many computational tasks whose result can easily be verified, and thus the provers do not need to be trusted.
In particular, the proof in Boojum is computed by recursively aggregating a very large number of smaller proofs (thousands to tens of thousands in a practical deployment).
Those are easy to verify by definition.

An important resource that can easily become a bottleneck for fast proof generation is also the bandwidth between different components of the system.
Given that the sizes of inputs and outputs of different tasks vary widely, bandwidth considerations are important.
For example, the size of a proof is, again by definition, small.
Thus, a proof can be easily transmitted over the internet.
On the other hand, inputs to provers could be, at some stages,
too large for internet transmission and the components generating them might need to be co-located with the provers.
Again, our system chooses the outsourced tasks such that both their inputs and their outputs are small.

Our main performance metric is end-to-end latency - the time between the sequencer outputting a batch and the prover outputting a valid proof. The cost of proving is the amount of money the rollup spends on running its own infrastructure and on paying external provers for their work. We evaluate our community prover with respect to both and quantify the trade-offs with respect to running a dedicated proving system for the rollup. Our results show that...

\subsection{Contributions}
This paper makes the following contributions.

\begin{enumerate}
    \item First, we design a community-based proving system, where the rollup operator is able to offload proving tasks to the community, via the introduction of a Job Distributor to the system.
    \item Second, we experimentally evaluate our system, and show that it match the performance of, and even outperform, the current deployment, even in systems of reasonable size and using consumer-grade hardware.
\end{enumerate}

==> results.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Circuit ID} & \textbf{120 GB (15 cores)} & \textbf{64 GB (8 cores)} & \textbf{32 GB (4 cores)} & \textbf{16 GB (2 cores)} \\ \hline
1   & (71.008, 3) & (91.082, 3) & (146.286, 4) & (915.032, 3) \\ \hline
2   & (81.586, 1) & (103.151, 2) & (163.442, 1) & (975.388, 1) \\ \hline
3   & (65.415, 3) & (80.232, 3) & (123.971, 4) & (794.692, 3) \\ \hline
4   & (81.444, 3) & (103.318, 3) & (153.979, 4) & (930.317, 3) \\ \hline
5   & (54.780, 3) & (69.707, 3) & (106.781, 4) & (551.604, 3) \\ \hline
6   & --          & (87.148, 1) & --           & --          \\ \hline
7   & (59.964, 3) & (77.690, 3) & (111.359, 4) & (630.464, 3) \\ \hline
8   & (87.494, 1) & (106.229, 3) & (158.500, 1) & (973.257, 1) \\ \hline
9   & (90.808, 3) & (112.258, 3) & (180.718, 4) & (992.291, 3) \\ \hline
10  & (66.746, 3) & (83.957, 3) & (122.918, 4) & (785.187, 3) \\ \hline
11  & (71.642, 1) & (87.255, 1)  & (158.044, 1) & --          \\ \hline
12  & --          & (90.102, 1)  & --           & --          \\ \hline
13  & (76.571, 1) & --           & --           & --          \\ \hline
255 & (59.700, 2) & (76.919, 1)  & (111.416, 1) & --          \\ \hline
\end{tabular}
\caption{Average time in seconds for different circuits across compute-optimized CPUs (C2) with 120 GB, 64 GB, 32 GB, and 16 GB architectures}
\label{table:time_comparison_extended}
\end{table}


\begin{table}[ht!]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Cores} & \textbf{16 GB} & \textbf{32 GB} & \textbf{64 GB} \\ \hline
CPU, 16 & -- & 67.7 ± 2.1 & 93.7 ± 1.9 \\ \hline
CPU, 8  & 421.8 ± 37.0 & 97.6 ± 3.1 & 116.5 ± 18.7 \\ \hline
CPU, 4  & -- & 148.2 ± 4.0 & -- \\ \hline
GPU, 4  & -- & 14.4 & -- \\ \hline
\end{tabular}
\caption{Average proving times in seconds for Circuit ID 1 across different RAM and core configurations}
\label{table:proving_times_circuit_1}
\end{table}
